AutoBalance: Optimized Loss Functions for Imbalanced Data

Imbalanced datasets are commonplace in modern machine learning problems. The presence of under-represented classes or groups with sensitive attributes results in concerns about generalization and fairness. Such concerns are further exacerbated by the fact that large capacity deep nets can perfectly fit the training data and appear to achieve perfect accuracy and fairness during training, but perform poorly during test. To address these challenges, we propose AutoBalance, a bi-level optimization framework that automatically designs a training loss function to optimize a blend of accuracy and fairness-seeking objectives. Specifically, a lower-level problem trains the model weights, and an upper-level problem tunes the loss function by monitoring and optimizing the desired objective over the validation data. Our loss design enables personalized treatment for classes/groups by employing a parametric cross-entropy loss and individualized data augmentation schemes. We evaluate the benefits and performance of our approach for the application scenarios of imbalanced and group-sensitive classification. Extensive empirical evaluations demonstrate the benefits of AutoBalance over state-of-the-art approaches. Our experimental findings are complemented with theoretical insights on loss function design and the benefits of train-validation split. All code is available open-source.

==> sec/fisher.tex <==
%\section{Consistent Logit Adjustment for Groups}
\section{Fisher Consistency of Logit Adjustment for Groups}
Consider the (class, group)-personalized logit adjustment loss function
\begin{align}
	%\ell(y,f(\x))=-w_{yg}\log\left(\frac{e^{\sigma(\Delta_{yg})f_y(\x)+l_{yg}}}{\sum_{i\in[K]}e^{\sigma(\Delta_{ig})f_i(\x)+l_{ig}}}\right).\label{la loss}
	\ell(y,f(\x))=-w_{yg}\log\left(\frac{e^{f_y(\x)+l_{yg}}}{\sum_{i\in[K]}e^{f_i(\x)+l_{ig}}}\right).\label{la loss}
\end{align}
%Recall the (class, group) balanced risk .
%Note that, this loss is a special case of the more general loss (which is also the group generalization of \eqref{AB loss})
%\begin{align}
%\ell(y,f(\x))=-w_{yg}\log\left(\frac{e^{\sigma(\Delta_{yg})f_y(\x)+l_{yg}}}{\sum_{i\in[K]}e^{\sigma(\Delta_{ig})f_i(\x)+l_{ig}}}\right).\label{AB loss gen}
%\end{align}
The following result guarantees consistency for the (class, group)-balanced loss $\Dtb$. The proof is in similar spirit to the proof of Theorem 1 in \cite{menon2020long}.
\begin{lemma} Let $\Dtb$ be the group-balanced distribution obtained by equally weighting $(\Dc_{k,j})_{(k,j)\in [K]\times [G]}$. For any $\bota\in\R^{K\times G}$, Group-LA loss \eqref{la loss} with the following weight choice is Fisher consistent for the (class, group)-balanced error $\Dtb$
\[
w_{kj}=e^{l_{kj}}/\bpi_{kj}\quad\text{for}\quad (k,j)\in [K]\times[G].%\tpi_{j}
\]
Specifically, when $w_{kj}=1$, $l_{kj}=\log\bpi_{kj}$ is a valid Group-LA loss.
\end{lemma}

\begin{proof} Denote the labeling likelihood $\eta_{yg}(\x)=\P(y\bgl \x)$. Observe that, when $w_{kj}=1$, the Bayes-optimal function minimizing the cross-entropy risk 
\[
\E[\ell_{\bota}(y,\x)]=-\sum_{g\in[G]}\E[\log\left(\frac{e^{f_y(\x)+l_{yg}}}{\sum_{i\in[K]}e^{f_i(\x)+l_{ig}}}\right)\Pro(g)]
\]
where the $\log\left(\frac{e^{f_y(\x)+l_{yg}}}{\sum_{i\in[K]}e^{f_i(\x)+l_{ig}}}\right)$ term has the conditional $(\x,y)|g$ distribution.

\SO{Questions:\\
1.~Does it become easier if $\x$ is independent of $g$?\\
2.~Is group-weighted xent consistent?}


The optimal decision rule is given by $f^*_y(\x)+l_{yg}=\log\eta_{yg}(\x)$.  This leads to the decision rule $f^*_y(\x)=\log\frac{\eta_{yg}(\x)}{e^{l_{yg}}}$. With multiplicative $\Delta$, decision rule becomes 
\[
f^*_y(\x)=\log(\frac{\eta_{y}(\x)}{e^{l_{y}}})^{\Delta_{y}^{-1}}
\]
\[
\arg\max_{y}\eta_y(\x)^{\Delta_y}=\arg\max_y c_y\eta_y(\x).
\]
Note that, the decision rule $f^*_y(\x)=\log\frac{\eta_{yg}(\x)}{\bpi_{yg}}$ is the decision rule for the Bayes-optimal classifier minimizer group-balanced error. The reason is that, $\frac{\eta_{yg}(\x)}{\bpi_{yg}}$ is proportional to the labeling function for the group-balanced distribution $\Dtb$.

\[
P(y|\x)=\frac{P(\x|y)P(y)}{\sum_{k=1}^K P(\x|k)P(k)}\implies \frac{P(y|\x)}{P(y)}=\frac{P(\x|y)}{\sum_{k=1}^K P(\x|k)P(k)}
\]

Let $\bpit_g\propto w_g\tpi_g$ be the $\w$-adjusted group-conditional distribution induced by $\w$-scaling the entries of group-conditional probabilities $\tpi$. The expected risk obeys
\begin{align}
\E_{\Dc}[\ell_{\w,\bota}(y,f(\x))]&=\sum_{g\in [G]}\tpi_{g}\cdot \E_{\Dt_g}[\ell_{\w,\bota}(y,f(\x))]\\
&=\sum_{g\in [G]}w_{g}\tpi_{g}\cdot \E_{\Dt_g}[\ell_{\bota}(y,f(\x))]\\
&\propto\sum_{g\in [G]}\bpit_{g}\cdot \E_{\Dt_g}[\ell_{\bota}(y,f(\x))].
\end{align}
Thus, LA loss with weights $\w$ is equivalent to LA-loss with flat $\w$ with adjusted probabilities $\bpit$.
\end{proof}
